Setting the Record Straight on Transformer Oversmoothing

Transformer-based models have recently become wildly successful across a diverse set of domains. At the same time, recent work has shown empirically and theoretically that Transformers are inherently limited. Specifically, they argue that as model depth increases, Transformers oversmooth, i.e., inputs become more and more similar. A natural question is: How can Transformers achieve these successes given this shortcoming? In this work we test these observations empirically and theoretically and uncover a number of surprising findings. We find that there are cases where feature similarity increases but, contrary to prior results, this is not inevitable, even for existing pre-trained models. Theoretically, we show that smoothing behavior depends on the eigenspectrum of the value and projection weights. We verify this empirically and observe that the sign of layer normalization weights can influence this effect. Our analysis reveals a simple way to parameterize the weights of the Transformer update equations to influence smoothing behavior. We hope that our findings give ML researchers and practitioners additional insight into how to develop future Transformer-based models.

==> figures/condition_number.tex <==
\begin{figure}[h!]
\centering

% \subcaptionbox{\textbf{Asymmetry of the matrix $\rmH$.})}{
% \includegraphics[width=0.48\textwidth]{figures/asymW.pdf}} \hfill
% \subcaptionbox{\textbf{Condition number of the matrix $\rmH$.}}{
\includegraphics[width=0.48\textwidth]{figures/condW.pdf} 
% $\frac{\|\mathrm{HFC}[\rmX_\ell]\|_2}{\|\mathrm{LFC}[\rmX_\ell]\|_2}$ and 
\caption{The average condition number of all $\rmH$ for ViT-Ti throughout training on CIFAR100.}
\label{fig:condition_number}
\end{figure}

==> figures/filtering.tex <==
\begin{figure*}[t]
\centering
% \subcaptionbox{Low-pass filter}{
% \includegraphics[width=0.9\textwidth]{figures/diffusion_steps_pos.png}
% }
% \subcaptionbox{High-pass filter}{
% \includegraphics[width=0.9\textwidth]{figures/diffusion_steps_neg.png}
% }
\includegraphics[width=0.9\textwidth]{figures/oversmoothing_visualization.png}
\caption{\textbf{Transformers can oversmooth, or not.} Evolution of the system $\rmX_{\ell} = \rmX_{\ell-1}+ \rmA \rmX_{\ell-1}\rmW_V\rmW_{\mathsf{proj}}$. When $\rmA$ has its most positive eigenvalue dominate $\eigAone$ we get oversmoothing. If instead its smallest eigenvalue dominates $\eigAn$, we get sharpening.}
\label{fig:filtering}
\end{figure*}

==> figures/frequency_ratio.tex <==

% \setlength\intextsep{0pt}
% \begin{wrapfigure}[19]{r}{0.4\textwidth}
% \vspace{-3ex}
\begin{figure}[t!]%{\columnwidth}

\centering
%\vspace{-6ex}
\includegraphics[width=\columnwidth]{figures/cifar100_filtering_last_layer.pdf}
\caption{\textbf{Filtering during training.} $\frac{\|\mathrm{HFC}[\rmX_\ell]\|_2}{\|\mathrm{LFC}[\rmX_\ell]\|_2}$ of the last layer for CIFAR100 models during training.} %We use $Asym(X) = \frac{\|(X-X^\top)/2\|_F}{\|(X+X^\top)/2\|_F}$ as a measure of symmetry. The matrix $\rmW_V \rmW_{proj}$ becomes more symmetric during training.}
%\vspace{-6ex}
\label{fig:ratio}
\end{figure}

==> figures/norm_impact.tex <==
\begin{figure}
  \centering
  \subcaptionbox{Impact of Pre-Norm and Post-LN on a smoothing layer}{
    \centering
    \includegraphics[width=.4\linewidth]{figures/smoothing_norm_impact.pdf} % Replace with your image filename
  }
  \subcaptionbox{Impact of Pre-Norm and Post-LN on a sharpening layer}{
    \centering
    \includegraphics[width=.4\linewidth]{figures/sharpening_norm_impact.pdf} % Replace with your image filename
  }
  \caption{\textbf{Pre-LN can change a layer's behavior}: We measure $\frac{\|\mathrm{HFC}[\rmX_\ell]\|_2}{\|\mathrm{LFC}[\rmX_\ell]\|_2}$ when applying a smoothing and sharpening layer for 128 iterations. The filterin behavior of the layer can be reversed when Pre-LN is used and the weights are negative} % Overall caption
  \label{fig:main}
\end{figure}

==> figures/similarity.tex <==
\begin{figure}[t!]
\centering
% \subcaptionbox{CIFAR100 (random init)}{
% \includegraphics[width=0.32\textwidth]{figures/similarity_random.pdf}
% } \hfill
% \subcaptionbox{ImageNet (random)}{
% \includegraphics[width=0.48\textwidth]{figures/similarity_random_imagenet.pdf}}
% \subcaptionbox{CIFAR100 (trained)}{
\includegraphics[width=\columnwidth]{figures/cifar100_filtering.pdf}
% } \hfill
% \subcaptionbox{ImageNet (trained)}{
% \includegraphics[width=0.32\textwidth]{figures/similarity_imagenet.pdf}
% }
\caption{\textbf{Filtering, image classification.} $\frac{\|\mathrm{HFC}[\rmX_\ell]\|_2}{\|\mathrm{LFC}[\rmX_\ell]\|_2}$ for different models on CIFAR100.}
\label{fig:dirichlet}
\end{figure}

==> figures/similarity_crammed_bert.tex <==
\begin{figure}[t!]%{r}{0.5\textwidth}
% \vspace{-3ex}
\centering
\includegraphics[width=\columnwidth]{figures/crammed_bert_filtering.pdf}
\caption{\textbf{Filtering, text generation.} $\frac{\|\mathrm{HFC}[\rmX_\ell]\|_2}{\|\mathrm{LFC}[\rmX_\ell]\|_2}$ for different models on The Pile.}
\label{fig:filtering_nlp}
%\vspace{-8.5ex}
\end{figure}

==> figures/symmetry.tex <==

% \setlength\intextsep{0pt}
% \begin{wrapfigure}[19]{r}{0.4\textwidth}
\begin{wrapfigure}{r}{0.4\textwidth}
\vspace{-3ex}
\centering
% \vspace{-0.5cm}
\includegraphics[width=\linewidth]{figures/asymW.pdf}
\caption{\textbf{Asymmetry of the matrix $\rmH := \rmW_{\mathsf{proj}}^\top\rmW_V^\top $, measured as $\frac{\| (\rmH - \rmH^\top)  / 2\|}{\| (\rmH + \rmH^\top) / 2\| }$.}} %We use $Asym(X) = \frac{\|(X-X^\top)/2\|_F}{\|(X+X^\top)/2\|_F}$ as a measure of symmetry. The matrix $\rmW_V \rmW_{proj}$ becomes more symmetric during training.}
%\vspace{-5ex}
\label{fig:symmetry}
\end{wrapfigure}

==> figures/text_depth.tex <==
\begin{figure*}[t]
\centering
% \subcaptionbox{Low-pass filter}{
% \includegraphics[width=0.9\textwidth]{figures/diffusion_steps_pos.png}
% }
% \subcaptionbox{High-pass filter}{
% \includegraphics[width=0.9\textwidth]{figures/diffusion_steps_neg.png}
% }
\vspace{-3ex}
\includegraphics[width=\textwidth]{figures/crammed_bert_test.pdf}
\vspace{-4ex}
\caption{\textbf{Text generation.} The test performance results on SuperGlue tasks for models with $\{16,32\}$ layers.}
\label{fig:superglue_depth}
\end{figure*}

==> figures/vision_depth.tex <==
\begin{figure*}[t]
\centering
% \subcaptionbox{Low-pass filter}{
% \includegraphics[width=0.9\textwidth]{figures/diffusion_steps_pos.png}
% }
% \subcaptionbox{High-pass filter}{
% \includegraphics[width=0.9\textwidth]{figures/diffusion_steps_neg.png}
% }
\includegraphics[width=\textwidth]{figures/cifar100_depth_bars_both.pdf}
\vspace{-4ex}
\caption{\textbf{Image classification.} The train and test error results on CIFAR100 for models with $\{12,24,48\}$ layers.}
\label{fig:cifar100_depth}
\end{figure*}

==> sections/5_experiments.tex <==
\label{sec:experiments}

==> sections/6_discussion.tex <==
\label{sec:discussion}

==> tables/conditions.tex <==
\begin{table*}[t!]
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|ccc|cccc|ccc}
        \toprule
        & \multicolumn{3}{c|}{ CIFAR100} & \multicolumn{4}{c|}{ ImageNet } & \multicolumn{3}{c}{ The Pile } \\
        \midrule
        Model & ViT-Ti & \textcolor{MidnightGreen}{ViT-Ti (sharpening)} & \textcolor{Rufous}{ViT-Ti (smoothing)} & ViT-B & DeiT-B & ViT-L & DeiT3-L & Cram. Bert & \textcolor{MidnightGreen}{Cram. Bert (sharpening)} & \textcolor{Rufous}{Cram. Bert (smoothing)} \\
        \midrule
        $(1 + \lambda^H_j \eigAn)$ & 73.99\% & 0\% & 100\% & 77.95\% & 99.05\% & 71.67\% & 100\% & 90\% & 0\% & 100\% \\
        $(1 + \lambda^H_j \eigAone)$ & 26.01\% & 100\% & 0\% & 22.05\% & 00.94\% & 28.33\% & 0\% & 10\% & 100\% & 0\%  \\
        \bottomrule
        \end{tabular}
        }
    \caption{\textbf{Distribution of dominating eigenvalues.} We compare different vision models trained on CIFAR100 and language models trained on The Pile, and count the percentage of cases where the dominating eigenvalue is $(1 + \lambda^H_j \eigAn)$ or $(1 + \lambda^H_j \eigAone)$.} 
    \label{tab:eigenvalues}
\end{table*}

%\cite{wang2022anti}
% \cite{ali2023centered}

==> tables/corrupted.tex <==
\begin{table*}[t]
        \centering
        \resizebox{\textwidth}{!}{
        \begin{tabular}{c|ccccccc}
        \toprule
        \bf Corruption Intensity & 0 & 1 & 2 & 3 & 4 & 5 \\
        \midrule
        ViT-Ti & $66.78_{\pm 0.1}$ & $61.59_{\pm 0.2}$ & $57.75_{\pm 0.2}$ & $53.12_{\pm 0.1}$ & $49.32_{\pm 0.1}$ & $39.17_{\pm 0.2}$ \\
        ViT-Ti + Featscale & $66.57_{\pm 0.5}$ & $61.25_{\pm 0.5}$ & $57.36_{\pm 0.6}$ & $52.64_{\pm 0.6}$ & $48.87_{\pm 0.5}$ & $38.77_{\pm 0.4}$ \\
        \midrule
        ViT-Ti$^+$ & $64.34_{\pm 0.3}$ & $58.36_{\pm 0.4}$ & $53.83_{\pm 0.5}$ & $49.03_{\pm 0.6}$ & $45.15_{\pm 0.6}$ & $35.86_{\pm 0.6}$ \\
        ViT-Ti$^-$ & $66.62_{\pm 0.3}$ & $61.62_{\pm 0.2}$ & $58.00_{\pm 0.3}$ & $53.56_{\pm 0.2}$ & $49.70_{\pm 0.3}$ & $40.07_{\pm 0.2}$ \\
        ViT-Ti$^*$ & ${67.84_{\pm 0.6}}$ & ${62.49_{\pm 0.5}}$ & ${58.82_{\pm 0.7}}$ & ${54.32_{\pm 0.7}}$ & ${50.40_{\pm 0.6}}$ & ${40.38_{\pm 0.7}}$ \\
        ViT-Ti-NS$^-$ & $67.80_{\pm 0.2}$ & $\mathbf{63.03_{\pm 0.2}}$ & $\mathbf{59.65_{\pm 0.1}}$ & $\mathbf{55.05_{\pm 0.3}}$ & $\mathbf{51.30_{\pm 0.1}}$ & $\mathbf{41.33_{\pm 0.1}}$\\
        ViT-Ti-NS$^*$ & $\mathbf{68.53_{\pm 0.6}}$ & $\mathbf{63.01_{\pm 0.1}}$ & $\mathbf{59.44_{\pm 0.3}}$ & $\mathbf{54.90_{\pm 0.4}}$ & $\mathbf{51.12_{\pm 0.4}}$ & $40.90_{\pm 0.4}$\\

        \bottomrule
        \end{tabular}}

    \caption{\textbf{Corruption Robustness.} Test accuracy for different corruption intensities on CIFAR100.} 
     \label{tab:corrupted}
\end{table*}



==> tables/depth.tex <==
\begin{table*}[t]
        \begin{minipage}{0.32\textwidth}
        \begin{tabular}{c|cc}
        \toprule
        \bf Depth & 12 & 24 \\
        \midrule
        ViT-Ti & $66.78_{\pm 0.1}$ & $67.22_{\pm 0.1}$\\
        \midrule
        ViT-Ti$^-$ & $66.62_{\pm 0.3}$ & $66.76_{\pm 0.3}$ \\
        ViT-Ti$^*$ & $67.84_{\pm 0.6}$ & $69.05_{\pm 0.1}$ \\
        ViT-Ti-NS$^-$ & $67.80_{\pm 0.2}$ & $67.09_{\pm 0.1}$\\
        ViT-Ti-NS$^*$ & $\mathbf{68.53_{\pm 0.6}}$ & $\mathbf{69.64_{\pm 0.3}}$\\
        % ViT-Ti$^.$ & $66.62_{\pm 0.003}$ & $66.96$ & $66.22$\\
        \bottomrule
        \end{tabular}
        

    \caption{\textbf{Increased Depth.} Results for different model depths on the CIFAR100 dataset  
     \label{tab:depth}}
     \end{minipage}
\end{table*}

% \begin{table*}[t]
%         \begin{minipage}{0.32\textwidth}
%         \begin{tabular}{c|ccc}
%         \toprule
%         \bf Depth & 12 & 24 & 48 \\
%         \midrule
%         ViT-Ti & $66.78_{\pm 0.1}$ & $67.22_{\pm 0.1}$ & $67.49_{\pm 0.2}$\\
%         \midrule
%         ViT-Ti$^+$ & $64.34_{\pm 0.3}$ & $65.37$ & $66.28$\\
%         ViT-Ti$^-$ & $66.62_{\pm 0.3}$ & $66.54$ & $66.54$\\
%         ViT-Ti$^*$ & $\mathbf{67.84_{\pm 0.6}}$ & $\mathbf{69.05_{\pm 0.1}}$ & $\mathbf{68.2_{\pm 0.6}}$\\
%         % ViT-Ti$^.$ & $66.62_{\pm 0.003}$ & $66.96$ & $66.22$\\
%         \bottomrule
%         \end{tabular}
        

%     \caption{\textbf{Increased Depth.} Results for different model depths on the CIFAR100 dataset  
%      \label{tab:depth}}
%      \end{minipage}
% \end{table*}

==> tables/lowdata.tex <==
\begin{table*}[t]
        \begin{minipage}{0.62\textwidth}
        \begin{tabular}{c|ccc}
        \toprule
        \bf Data kept & 100\% & 50\% & 10\% \\
        \midrule
        ViT-Ti & $66.78_{\pm 0.1}$ & $56.38_{\pm 0.5}$ & $32.47_{\pm 0.9}$\\
        ViT-Ti + FeatScale & $66.57_{\pm 0.5}$ & $57.08_{\pm 0.3}$ & $32.50_{\pm 0.4}$\\
        \midrule
        ViT-Ti$^+$ & $64.34_{\pm 0.3}$ & $55.21_{\pm 0.5}$ & $28.67_{\pm 0.5}$\\
        ViT-Ti$^-$ & $66.62_{\pm 0.3}$ & $56.58_{\pm 0.3}$ & $\mathbf{33.99_{\pm 0.4}}$\\
        ViT-Ti$^*$ & $\mathbf{67.84_{\pm 0.6}}$ & $\mathbf{57.78_{\pm 0.4}}$ & $\mathbf{33.64_{\pm 0.5}}$\\
        ViT-Ti-NS$^-$ & $67.80_{\pm 0.2}$ & $57.54_{\pm 0.1}$ &  \\
        ViT-Ti-NS$^*$ & $68.53_{\pm 0.6}$ & $57.67_{\pm 0.3}$ & $33.75_{\pm 0.2}$ \\
        \bottomrule
        \end{tabular}
        

        \caption{\textbf{Data Efficiency.} Results for different percentages of the CIFAR100 used in training.} 
         \label{tab:efficiency}
         \end{minipage}
\end{table*}

==> tables/nanogpt.tex <==
\begin{wraptable}{r}{0.45\textwidth}
% \vspace{-0.5ex}
% \begin{table}[!ht]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{l|l|l}
    \toprule
        Model & MiniPile & Shakespeare \\ 
    \midrule
        NanoGPT-Ti & $\mathbf{21.864}$ & $\mathbf{62.084}$ \\ 
    \midrule
        NanoGPT-Ti-NS$^+$  & 25.442 & 71.870 \\ 
        NanoGPT-Ti-NS$^-$  & 24.436 & 67.067 \\ 
        NanoGPT-Ti-NS$^*$  & 22.968 & 64.599 \\ 
    \bottomrule
    \end{tabular}
    }
    \caption{\textbf{NLP results.} Perplexity on a Minipile held-out set and the Shakespeare dataset.}
    \label{tab:nanogpt}
% \vspace{-8ex}

\end{wraptable}


==> tables/vision.tex <==
\begin{table*}[t!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{c|cccccccccc}
    \toprule
     & \multicolumn{2}{c}{ViT-Ti} & \multicolumn{2}{c}{ViT-Ti + FeatScale} & \multicolumn{2}{c}{ViT-Ti + Centered Attention} & \multicolumn{2}{c}{ViT-Ti$^-$} & \multicolumn{2}{c}{ViT-Ti$^+$} \\
     \midrule
    Depth & Train & Test & Train & Test & Train & Test & Train & Test & Train & Test \\
    \midrule
    12 & $92.17_{\pm  0.002}$ & $68.71_{\pm  0.08}$ & $92.29_{\pm  0.444}$ & $68.95_{\pm  0.415}$ & $91.06_{\pm  0.222}$ & $66.6_{\pm  0.502}$ & $94.31_{\pm  0.23}$ & $70.74_{\pm  0.547}$ & $90.61_{\pm  0.576}$ & $70.3_{\pm  0.531}$ \\
    24 & $95.26 _{\pm  0.039}$ & $69.69_{\pm  0.31}$ & $95.13_{\pm  0.2}$ & $69.83_{\pm  0.0}$ & $94.01_{\pm  0.052}$ & $69.34_{\pm  0.095}$ & $96.95_{\pm  0.1}$ & $70.86_{\pm  0.17}$ & $94.32_{\pm  0.086}$ & $71.46_{\pm  0.301}$ \\
    48 &  & $69.17$ &  & $69.39$ &  &  &  & $70.98$ &  & $71.79$ \\
    \bottomrule
    \end{tabular}}
\caption{\textbf{Increased Depth.} Train and test accuracy for different model depths on CIFAR100.} 
\label{tab:vision_results}

\end{table*}







